Learning to Infer Program Sketches

Our goal is to build systems which write code automatically from the kinds of specifications humans can most easily provide, such as examples and natural language instruction. The key idea of this work is that a flexible combination of pattern recognition and explicit reasoning can be used to solve these complex programming problems. We propose a method for dynamically integrating these types of information. Our novel intermediate representation and training algorithm allow a program synthesis system to learn, without direct supervision, when to rely on pattern recognition and when to perform symbolic search. Our model matches the memorization and generalization performance of neural synthesis and symbolic search, respectively, and achieves state-of-the-art performance on a dataset of simple English description-to-code programming problems.

==> ICML2019 Arxiv (camera ready) copy/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICML2019 Arxiv (camera ready) copy/supp_text.tex <==

\section{Architecture Details}
\textbf{Generator:}

Our Generator neural network architecture is nearly identical to the ÒAttn-AÓ RobustFill model \citep{devlin2017robustfill}. This is a sequence-to-sequence model which attends over multiple input-output pairs.
%The network consists of three separate LSTMs: an input encoder $I$, an output encoder $O$, and a program decoder $P$. A separate copy of the network encodes each input-output example, and the results are maxpooled in order to decode a program. Each input-output example is encoded as follows: the input example is encoded by $I$. The output example is encoded by $O$ while attending to $I$. TODO FINISH
Our model differs from the ÒAttn-AÓ RobustFill model by adding a learned grammar mask. As in \citet{bunel2018leveraging}, we learn a separate LSTM language model over the program syntax. The output probabilities of this LSTM are used to mask the output probabilities of the Generator model, encouraging the model to put less probability mass on grammatically invalid sequences. 

For the Algolisp experiments, we did not condition the Generator on input-output examples, instead encoding the natural language descriptions for each program. In these experiments, the Generator is simply a sequence-to-sequence LSTM model with attention, coupled with a learned grammar mask, as above.

For the Generator model, \textbf{HOLE} is simple an additional token added to the program DSL. During training, sketches are sampled via Equation 6 in the main text, and are converted to a list of tokens to be processed by the Generator, as is typical with RNN models.

\textbf{Recognizer:}

The recognizer model consists of an LSTM encoder followed by a feed-forward MLP. To encode a specification, each input-output example is separately tokenized (a special \code{EndOfInput} token is used to separate input from output), and fed into the LSTM encoder. The resulting vectors for each input-output example are averaged. The result is fed into the feed-forward MLP, which terminates in a softmax layer, predicting a distribution over output production probabilities.

This architecture differs slightly from the DeepCoder model \citep{balog2016deepcoder}, which encodes inputs and outputs via a feedforward deep network without recurrence. However, the models are similar in functionality; both models encode input-output specs, average the hidden vectors for each example, and decode a distribution over production probabilities. Both models use the resulting distribution to guide a symbolic enumerative search over programs. Our enumeration scheme is equivalent to the depth first search experiments in \citet{balog2016deepcoder}.

For the Algolisp experiments, we did not condition the Recognizer on input-output examples, instead encoding the natural language descriptions for each program. In these experiments, the LSTM encoder simply encodes the single natural language specification and feeds it to the MLP. As in the other domains, the examples are still used by the synthesizer to determine if enumerated candidate programs satisfy the input-output specification.

\section{Experimental details}
All code was written in Python, and neural network models were implemented in PyTorch and trained on NVIDIA Tesla-x GPUs. All networks were trained with the Adam optimizer \citep{kingma2014adam}, with a learning rate of 0.001. Our sketch generator LSTMs used embedding sizes of 128 and hidden sizes of 512. Our recognizer networks used LSTMs with embedding sizes of 128, hidden sizes of 128, and MLPs had a single hidden layer of size 128. For all domains, we trained using a timeout parameter $t$ sampled from $t \sim \text{Exp}(\alpha)$, where $\alpha=0.25$.

\subsection{List Processing}

\textbf{Data:}
We use the test and training programs from \citet{balog2016deepcoder}. The test programs are simply all of the length $N$ programs, pruned for redundant or invalid behavior, for which there does not exist a smaller program with identical behavior. We converted these programs into a $\lambda$-calculus form to use with our synthesizer.

As in \citet{balog2016deepcoder}, input-output example pairs were constructed by randomly sampling an input example and running the program on it to determine the corresponding output example. We used simple heuristic constraint propagation code, provided to us by the authors of \citet{balog2016deepcoder}, to ensure that sampled inputs did not cause errors or out-of-range values when the programs were run on them.

\textbf{Training:}
For the sketch generator, we used a batch size of 200. We pretrained all sketch generators on the full programs for 10 epochs, and then trained on our sketch objective for 10 additional epochs. 
We also note that, we trained the RNN baseline for twice as long, 20 epochs, and observed no difference in performance from the baseline trained for 10 epochs.  The Deepcoder-style recognizer network was trained for 50 epochs.
%
%For length = 4:\\
%We pretrained all sketch generators on full programs for 8000 batches and then trained them on our sketch objective for an additional 5000 batches.
%We trained the Deepcoder-style recognizer network on the entire training set once, about 11 million programs.

The sketch Generator models had approximately 7 million parameters, and the Recognizer model had about 230,000 parameters.

\subsection{String Transformations}

\textbf{Data:}
As our DSL, we use a modified version of the string transformation language in \citet{devlin2017robustfill}. Because our enumerator uses a strongly typed  $\lambda$-calculus, additional tokens, such as \code{concat\_list}, \code{concat1}, \code{expr\_n} and \code{delimiter\_to\_regex} were added to the DSL to express lists and union types.

\textbf{Training:}
Our Generator and Recognizer networks were each trained on 250,000 programs randomly sampled from the DSL. The sketch Generator used a batch size of 50.

\subsection{AlgoLisp}
\textbf{Data:}
We implemented \system{} and our baselines for the AlgoLisp DSL in \citet{polosukhin2018neural}. As in \citet{bednarek2018ain}, we filter out evaluation tasks for which the reference program does not satisfy the input-output examples.

\textbf{Training:}
For the AlgoLisp domain, we used a batch size of 32, and trained our Generator and Recognizer networks until loss values stopped decreasing on the `dev' dataset, but for no fewer than 1250 training iterations.

\section{Additional Experimental Analysis}

\textbf{Training and testing with noisy specification:}
For the string editing domain---where real-world user input can often be noisy---we conducted an experiment to examine our system's performance when specifications have errors. we injected random noise (insertion, deletion, or substitution) into the training and testing data. We assume that only one of the test examples is corrupted, and measure the number of specs for which we can satisfy at least three out of four test examples. We report accuracy of 53\% for SketchAdapt, 52\% for ``Generator only", and 52\% for ``Synthesizer only". These results indicate that our system is affected by noise, but can still often recover the desired program from noisy inputs.

\textbf{Algolisp results using only IO specification:}
To determine the utility of the natural language descriptions in the Algolisp experiments, we report an additional ablation, in which the description is not used. In these experiments, the Generator and Recognizer networks are conditioned on the input-output examples instead of the program descriptions. Table \ref{algolispIOtable} reports our results for this ``IO only" ablation. We observe that without the natural language descriptions, neither \system{} or the lesioned baselines are able to synthesize many of the test programs. 



\begin{table}
\vspace{-0.25cm}
\caption{Algolisp results using only input-output specification}
\label{algolispIOtable}
\begin{center}
\begin{tabular}{lllll}
\hline
\multirow{2}{*}{Model}&\multicolumn{2}{c}{Full dataset}&\multicolumn{2}{c}{Filtered\footnotemark[1]}\\
 &\multicolumn{1}{l}{(Dev)}&\multicolumn{1}{l}{{Test\bf}}&\multicolumn{1}{l}{(Dev)}&\multicolumn{1}{l}{{Test\bf}}\\ 
\hline 
\system{}, IO only&(4.9)&8.3&(5.6)&8.8\\
Generator, IO only&(5.8)&2.4&(6.4)&2.7\\
Synthesizer, IO only&(8.7)&7.1&(9.3)&7.8\\
\hline
%Seq2Tree+Search&(86.1)&85.8&-&-\\
\end{tabular}
\end{center}
%\vspace{-0.5cm}
\end{table}

\begin{table*}[h]
\caption{Solve times for Algolisp test programs, in seconds}
\label{solvetime}
\begin{center}
\begin{tabular}{rr|l|l|l|l|l}
%& 25th & median & 75th & 25th & median & 75th & 25th & median & 75th & 25th & median & 75th & 25th & median & 75th\\
\\
& &\multicolumn{5}{c}{Number of training programs used} \\
& & 2000 & 4000 & 6000 & 8000 & Full dataset\\
\hline
\hline
\multirow{3}{*}{\system} & 25th percentile & 25.3 & 30.5 & 24.8 & 23.0 & 34.7\\
& median & 37.3 & 46.8 & 38.5 & 36.6 & 55.2\\
& 75th percentile & 62.7 & 71.0 & 55.3 & 56.1 & 85.8\\
\hline
\multirow{3}{*}{Generator only} & 25th percentile & 51.1 & 31.8 & 21.8 & 26.4 & 28.2\\
& median & 57.8 & 41.2 & 33.7 & 39.2 & 41.8\\
& 75th percentile & 100.6 & 60.8 & 49.3 & 59.2 & 63.5\\
\hline
\multirow{3}{*}{Synthesizer only} & 25th percentile & 0.4 & 0.5 & 0.6 & 0.5 & 0.4\\
& median & 0.8 & 0.9 & 1.0 & 0.9 & 0.9\\
& 75th percentile & 1.3 & 1.5 & 2.2 & 1.6 & 3.6\\
\hline
\end{tabular}
\end{center}
\end{table*}

\footnotetext[1]{As in \citet{bednarek2018ain}, we filter the  test and dev datasets for only those tasks for which reference programs satisfy the given specs.}
\textbf{Evaluation runtime for Algolisp dataset:}
We report solve time for the Algolisp test data in Table \ref{solvetime}. 
We report 25th percentile, median, and 75th percentile solve times.
We note that, despite using both neural beam search and enumerative search, \system{} does not find programs significantly slower than the RNN ``Generator only" baseline.
We also note that the ``Synthesizer only" solve times are significantly faster because only a small proportion of the programs were solved.



\textbf{Breakdown of results:}
In order to gain further insight into how our system compares to baselines, for each test domain, we examine to what extent problems solved by \system{} are not solved by baselines, and visa versa.  Figures \ref{deepcoderbreakdown}, \ref{rbbreakdown} and \ref{algolispbreakdown} report the degree of overlap between problems solved by \system{} and the strongest baseline.


For all domains, a large proportion of problems are solved by \system{} and not solved by the baseline, while a much smaller proportion of problems are solved by the baseline but not solved by \system{}.


We additionally provide samples of programs which were solved by \system{} and not solved by the strongest baseline (Figures \ref{listsamples}, \ref{textsamples}, and \ref{Algolispsamples}).

%Samples of breakdowns at different points\\
%takeaways:\\
%list processing: longer programs\\
%algolisp and text: easier inference\\

\begin{table}[H]
\caption{Breakdown of results in the list processing domain (train on length 3 programs, test  on length 4 programs). We examine the proportion of programs solved after evaluating fewer than $10^4$ candidates. We compare \system{} to the ``Synthesizer only" model, which is the best performing baseline in this domain.}
\label{deepcoderbreakdown}
\begin{center}
\begin{tabular}{lllllll}
&& \multicolumn{5}{c}{Synthesizer Only}\\
\multirow{4}{*}{\rotatebox[origin=c]{90}{\system{}}} & & solved & failed & sum \\
\cline{3-4}
 & solved & 19\% & 24\% & 43\%\\
 & failed & 2\% & 55\% & 57\% \\
\cline{3-4}
 & sum & 21\% & 79\% & \\
 \\
\end{tabular}
%\begin{tabular}{lllllll}
%&& \multicolumn{5}{c}{Synthesizer Only}\\
%\multirow{4}{*}{\rotatebox[origin=c]{90}{SketchAdapt}} & & hit & miss & sum \\
%\cline{3-4}
% & hit & 47\% & 9\% & 56\%\\
% & miss & 9\% & 35\% & 44\% \\
%\cline{3-4}
% & sum & 56\% & 44\% & \\
%\end{tabular}
\end{center}
\end{table}

\begin{table}[H]
\caption{Breakdown of results in the text editing domain. We compare \system{} to the ``Generator only" model, which is the best performing baseline in this domain.}
\label{rbbreakdown}
\begin{center}
\begin{tabular}{lllllll}
\\
&& \multicolumn{5}{c}{Generator Only}\\
\multirow{4}{*}{\rotatebox[origin=c]{90}{\system{}}} & & solved & failed & sum \\
\cline{3-4}
 & solved & 55.2\% & 7.8\% & 63.0\%\\
 & failed & 2.0\% & 35.0\% & 37.0\% \\
\cline{3-4}
 & sum & 57.2\% & 42.8\% & \\
\end{tabular}
\end{center}
\end{table}

\begin{table}[H]
\caption{Breakdown of results on Algolisp test data (trained on 6000 programs). We compare \system{} to the ``Generator only" model, which is the best performing baseline in this domain.}
\label{algolispbreakdown}
\begin{center}
\begin{tabular}{lllllll}
\\
&& \multicolumn{5}{c}{Generator Only}\\
\multirow{4}{*}{\rotatebox[origin=c]{90}{\system{}}} & & solved & failed & sum \\
\cline{3-4}
 & solved & 45.3\% & 20.8\% & 66.1\%\\
 & failed & 7.2\% & 26.7\% & 33.9\% \\
\cline{3-4}
 & sum & 52.5\% & 47.5\% & \\
\end{tabular}
\end{center}
\end{table}


%\begin{table*}
%\caption{\system{} hits from AlgoLisp dataset}
%\label{algohits}
%\begin{center}
%\begin{tabular}{p{6cm}p{6cm}p{3cm}}
%\multicolumn{1}{c}{\bf Spec}&\multicolumn{1}{c}{\bf Sketch}&\multicolumn{1}{c}{\bf Hole}
%\\ \hline \\
%given numbers a and b , let c be the maximum of a and b , reverse digits in c , compute c &
%\code{( reduce ( reverse ( digits ( max a <HOLE> ) ) ) 0 ( lambda2 ( + ( * arg1 10 ) arg2 ) ) )}
%&Where \code{<HOLE>} $\to$ \code{b}\\
%\hline
%\end{tabular}
%\end{center}
%\vspace{-.6cm}
%\end{table*}

\begin{figure*}
\caption{Sketches and programs found by \system{} in list processing domain}
%List Processing: \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
$\text{[123, -105, 60, 122, 7, -54, 15, 2, 44, 7], [-50, 82, 88, -37, 111, 115, 108, -44, 96, 107]}\to \text{[-50, -105, 8, -37, 7]}$, \\
$\text{[115, -75, -36, 98, -114, -91, 22, 28, -35, -7], [22, -123, -101, -17, 118, 86, 2, -106, 88, -75] $\to$ [22, -123, -101, -34, -114]}$,\\
\dots
\\
\textbf{Sketch:}\\
\code{(ZIPWITH MIN input1 (ZIPWITH MIN (FILTER <HOLE1> <HOLE2>) input0))}\\
where\\ \code{<HOLE0>} $\to$ \code{isEVEN}\\
\code{<HOLE1>} $\to$ \code{(MAP INC input0)}
}
}\vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
$\text{[4, -7, -6, 2, -5, -7, 4, -4, 1, -5], [-4, 1, 7, -3, -2, -7, 1, 5, -2, 7] $\to$ [0, 1, -26, -2]}$,\\
$\text{[3, -6, -6, 4, 2, -7, -4, 2, -4, -1], [-5, -6, 4, -7, 0, 7, -7, -5, 4, 3] $\to$ [-3, 52, -16, -20]}$,\\
\dots
\\
\textbf{Sketch:}\\
\code{(ZIPWITH + (FILTER <HOLE0> <HOLE1>) (ZIPWITH * input1 input0))}\\
where\\ \code{<HOLE0>} $\to$ \code{isPOS}\\
\code{<HOLE1>} $\to$ \code{(MAP MUL4 input0)}
}
}\vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
$\text{[-1, 5, -6, 1, -4, -7, -3, 6, 4, -1], [-6, -4, 3, 4, 3, -3, 0, 3, 5, -3] $\to$ [2, 50, 45, 17, 25, 58, 9, 72, 41, 2]}$,\\
$\text{[-4, 0, -4, 1, 2, -2, 7, 2, -2, -4], [-5, 6, -1, -7, -5, -6, -3, -4, 7, -5] $\to$ [32, 36, 17, 2, 8, 8, 98, 8, 53, 32]}$,\\
\dots
\\
\textbf{Sketch:}\\
\code{(ZIPWITH <HOLE0> (MAP SQR <HOLE1>) (MAP SQR input0))}\\
where\\ \code{<HOLE0>} $\to$ \code{+}\\
\code{<HOLE1>} $\to$ \code{(ZIPWITH MAX input1 input0)}
}
}\vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
$\text{[69, -49, 117, 7, -13, 84, -48, -125, 6, -68], [112, -44, 77, -58, -126, -45, 112, 23, -92, 42] $\to$ [-9, -21, -7, -15]}$,\\
$\text{[0, -76, -85, 75, 62, -64, 95, -77, -78, -114], [-111, 92, -121, 108, 5, -22, -126, -40, 9, -115] $\to$ [-21, -39, -57]}$,\\
\dots
\\
\textbf{Sketch:}\\
\code{(FILTER <HOLE0> (MAP DIV2 (ZIPWITH MIN input0 <HOLE1>)))}\\
where\\ \code{<HOLE0>} $\to$ \code{isODD}\\
\code{<HOLE1>} $\to$ \code{(MAP DIV3 input1)}
}
}
%\vspace{0.1cm}\\
%\textbf{MISSES:}\vspace{0.05cm}\\
%\fbox{
%\parbox{\linewidth}
%{
%\textbf{Spec:}\\
%\\
%\textbf{Sketch:}\\
%\code{blah}\\
%where\\ \code{<HOLE>} $\to$ \code{BLAH}
%}
%}
\label{listsamples}
\end{figure*}


\begin{figure*}
\caption{Sketches and programs found by \system{} in text editing domain. Programs edited for readability.}
%Text Editing: \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
(('Lashanda' $\to$ 'Las'), ('Pennsylvania' $\to$ 'Pennsyl'), ('California' $\to$ 'Calif'), ('Urbana' $\to$ 'U'))\\
\textbf{Sketch:}\\
\code{(apply\textunderscore fn <HOLE1> (SubStr <HOLE2> <HOLE3>))}\\
where\\ \code{<HOLE1>} $\to$ \code{GetTokenWord-1}\\
\code{<HOLE2>} $\to$ \code{Position0}\\
\code{<HOLE3>} $\to$ \code{Position-5}\\
}
}\vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
(('Olague(California' $\to$ 'California'), ('621(Seamons' $\to$ 'Seamons'), ('Mackenzie(Dr(5(Park' $\to$ 'Park'), ('+174(077(Storrs' $\to$ 'Storrs'))\\
\textbf{Sketch:}\\
\code{(apply\textunderscore fn GetFirst\textunderscore PropCase3 (GetSpan right\textunderscore paren index-1 <HOLE> Alphanum <HOLE> End))}\\
where\\ \code{<HOLE1>} $\to$ \code{End}\\
\code{<HOLE2>} $\to$ \code{Index-1}\\
}
} \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Spec:}\\
(('Karrie' $\to$ 'Karri'), ('Jeanice' $\to$ 'Jeani'), ('Brescia' $\to$ 'Bresc'), ('Lango' $\to$ 'Lango'))\\
\textbf{Sketch:}\\
\code{(concat\textunderscore list <HOLE> GetFirst\textunderscore Lower4)}\\
where\\ \code{<HOLE>} $\to$ \code{GetTokenAlphanum0}\\
}
} \vspace{0.05cm}\\
\label{textsamples}
\end{figure*}

\begin{figure*}
\caption{Sketches and programs found by \system{} in AlgoLisp dataset}
%Algolisp: \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Description:}\\
given numbers a and b , let c be the maximum of a and b , reverse digits in c , compute c\\
\textbf{Sketch:}\\
\code{(reduce
(reverse (digits (max a <HOLE>))) 0
(lambda2 (+ (* arg1 10) arg2)))}\\
where\\ \code{<HOLE>} $\to$ \code{b}
}
} \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Description:}\\
you are given arrays of numbers a and c and a number b , your task is to compute number of values in a that are less than values on the same index in reverse of values in c bigger than b\\
\textbf{Sketch:}\\
\code{(reduce (map (range 0 (min (len a) (len (reverse (<HOLE> c (partial1 b >)))))) (lambda1 (if (< (deref a arg1) (deref (reverse (filter c (partial1 b >))) arg1)) 1 0))) 0 +)}\\
where\\ \code{<HOLE>} $\to$ \code{filter}
}
} \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Description:}\\
consider arrays of numbers a and b and a number c , only keep values in the second half of a , compute sum of first c values among values of a that are also present in b after sorting in ascending order\\
\textbf{Sketch:}\\
\code{(reduce (slice (sort (filter (slice a (/ (len a) 2) (len a)) (lambda1 (reduce (map b (partial0 arg1 ==)) false || )))) 0 c) 0 +)}\\
where\\ \code{<HOLE>} $\to$ \code{reduce}
}
} \vspace{0.05cm}\\
\fbox{
\parbox{\linewidth}
{
\textbf{Description:}\\
consider a number a and an array of numbers b , your task is to find the length of the longest subsequence of odd digits of a that is a prefix of b\\
\textbf{Sketch:}\\
\code{(reduce (<HOLE> a) 0 (lambda2 (if (== arg2 (if (< arg1 (len b)) (deref b arg1) 0)) (+ arg1 1) arg1)))}\\
where\\ \code{<HOLE>} $\to$ \code{digits}
}
}
\label{Algolispsamples}
\end{figure*}
%\textbf{Theoretical Justification:}\\
%CUT
%
%It is important to note that both components of our model are performing different types of search.
%The RNN-based sketch generator performs a beam search, which is slow, but can still be very effective because it is guided by patterns learned from the training data. On the other hand, the enumerative sketch synthesizer receives some  guidance from the learned recognizer, but is mostly guided by the syntax and semantics of the DSL. Therefore it performs a very fast but less targeted search. Our model essentially learns how to effectively trade off between these types of search.

